Integration-free Learning of Flow Maps

We present a method for learning neural representations of flow maps from time-varying vector field data. The flow map is pervasive within the area of flow visualization, as it is foundational to numerous visualization techniques, e.g. integral curve computation for pathlines or streaklines, as well as computing separation/attraction structures within the flow field. Yet bottlenecks in flow map computation, namely the numerical integration of vector fields, can easily inhibit their use within interactive visualization settings. In response, in our work we seek neural representations of flow maps that are efficient to evaluate, while remaining scalable to optimize, both in computation cost and data requirements. A key aspect of our approach is that we can frame the process of representation learning not in optimizing for samples of the flow map, but rather, a self-consistency criterion on flow map derivatives that eliminates the need for flow map samples, and thus numerical integration, altogether. Central to realizing this is a novel neural network design for flow maps, coupled with an optimization scheme, wherein our representation only requires the time-varying vector field for learning, encoded as instantaneous velocity. We show the benefits of our method over prior works in terms of accuracy and efficiency across a range of 2D and 3D time-varying vector fields, while showing how our neural representation of flow maps can benefit unsteady flow visualization techniques such as streaklines, and the finite-time Lyapunov exponent.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> method.tex <==
In this section, we first discuss the preliminary concepts required to understand our approach followed by the details of our approach.

\subsection{Background: Flow Map}
Flow map is an important mathematical tool that is utilized by numerous flow visualization techniques. To understand the concept of flow map let us consider a time-dependent flow field $f : \mathbb{R}^n \times \mathbb{R} \rightarrow \mathbb{R}^n$, where $f(\mathbf{x}(t), t)$ describes the vector at the spatial position $\mathbf{x} \in \mathbb{R}^n$ at time $t$. Then, the trajectory of a massless particles advected under the influence of the flow field $f$ is governed by the following ordinary differential equation:
\begin{equation}
\frac{d \mathbf{x}(t)}{d t} = f(\mathbf{x}(t),t) , \quad \mathbf{x}(t_0) = \mathbf{x_0},
\end{equation}
where $\mathbf{x_0}$ represents the initial position of particle at starting time $t_0$. A flow map is used to encode these trajectories. More specifically, a flow map encodes the final position of a massless particle advected under the influence of a flow field for a finite-time span T. Formally, a flow map for the flow field $f(\textbf{x}(t), t)$ is given by:

\begin{equation}
    \phi(\mathbf{x_0}, t_0, \tau): \mathbb{R}^n \times \mathbb{R} \times \mathbb{R} \rightarrow \mathbb{R}^n = \mathbf{x_0} + \int_{t_0}^{t_0+\tau} f(\mathbf{x}(t),t) dt,  
\end{equation}

where $\phi$ encodes the position of a particle seeded at spatial position $\mathbf{x_0}$ and time $t_0$ after being advected under the flow for a duration of $\tau$. In practice, flow maps are computed using numerical integration scheme making it a computationally expensive process. Thus, motivating the need for an alternative representations of flow map that can eliminate the need for the expensive numerical integration process.

\subsubsection{Flow Map Properties}
\label{sec:flowmap_properties}
In fluid dynamics, there are some basic properties that a flow map satisfies when the integration duration $\tau = 0$. We list these properties below :-
\begin{equation}
    \label{eq:identity}
    \phi(\mathbf{x}, t, 0) = \mathbf{x}
\end{equation}

\begin{equation}
    \label{eq:zero_tau_deriv}
    \frac{\partial \phi(\mathbf{x}, t, 0)}{\partial \tau} = f(\mathbf{x}, t)
\end{equation}
Eq.~\ref{eq:identity} refers to the identity property of flow map, which describes that any particle seeded at spatial position $\mathbf{x}$ and time $t$ must map to the same spatial position $\mathbf{x}$ when the integration duration $\tau = 0$. Additionally, Eq.~\ref{eq:zero_tau_deriv} describes that the partial derivative of the flow map when $\tau = 0$ is equivalent to the vector at the seed position. We argue that both Eq.~\ref{eq:identity} and \ref{eq:zero_tau_deriv} are essential properties of a flow map and any alternative flow map representation should exhibit these properties to be a valid representation.

\subsection{Background: Implicit Neural Representations}
INRs are a class of neural networks that accepts the positional coordinates of a given scalar/vector field as input and predicts the scalar/vector at the input position. In the recent years, INRs have been used in various field as an alternative representation. In this section, we discuss about the two most widely used variants of INRs.

\textbf{SIREN}
These are the class of neural networks that uses sinusoidal activation functions in a multi layer perceptron (MLP) network architecture. More specifically, for a given input position $x \in \mathbb{R}^n$, SIREN performs the following operations:-
\begin{equation}
    z_0(\mathbf{x}) = sin(W_0\mathbf{x}),
\end{equation}
\begin{equation}
    z_i(\mathbf{x}) = sin(W_i z_{i-1}(\mathbf{x})),
\end{equation}
\begin{equation}
    f_\theta(\mathbf{x}) = W_l z_{l-1}
\end{equation}
where, $z_0$ represents the positional encoding, $z_i$ is the output at the $i^{th}$ layer of the $l$ layer MLP and $W_i$ is the weight matrix that comprises of the parameters of the network.

\textbf{Localized Grid-SIREN}
A major drawback of a single MLP INR is its inability to scale to larger dataset. To overcome these challenges, another variant of INRs have been proposed in the literature that utilizes a coarse spatial grid of learnable frequencies to generate the positional encoding. These variants are designed to scale to larger dataset meanwhile significantly improving the training and inference times as compared to their MLP counterparts. More specifically, for a given input $\mathbf{x} \in \mathbb{R}^n$, the positional encoding can be generated by interpolating within the grid using the following operation:-
\begin{equation}
    z_0(\mathbf{x}) = sin(interp(\mathbf{x}, Z)),
\end{equation}
where interp corresponds to an interpolation of the frequencies defined at the locations of Z.

\subsection{Naive Neural Flow Map Representation}
SIRENs/Localized Grid-SIRENs with their powerful representational capabilities can be readily used as an alternative representation for flow maps. However, such naive adaptation would require us to tack-on the integration duration as a coordinate. Consequently, resulting in scalability issues in terms of model size and the amount of training data required because of the necessity to optimize over a $(n+2)$-dimensional space, where $n$ represents the spatial dimension of the flow field. Additionally, the default architectures do not satisfy the basic properties of identity mapping described in Eq.~\ref{eq:identity} by design. Thus, one has to enforce the identity mapping by introducing a regularization term during optimization. However, at best, this results in an identity approximation and not an exact identity mapping. Moreover, the resulting partial derivative of the neural flow map with respect to $\tau$ is also non-trivial. Thus, motivating the need for a better neural flow map architectural design. 

\subsection{Neural Flow Map Representation}
\label{sec:neural_flow_map}
In this section, we give the basic idea behind of our approach and how our proposed network architecture overcomes the short-comings of a naive INR network design. We aim to satisfy the following goals for our network design (1)
exhibit the basic properties of flow maps (c.f~\ref{sec:flowmap_properties}) and (2) allow the model to learn efficiently without requiring tremendous amount of data.

\subsubsection{Satisfying flow map properties}
\label{sec:learning_vf}
\begin{figure}[!t]
  \centering
 	\includegraphics[width=\linewidth]{figures/approach-overview.pdf}
	\caption{TODO}
    \label{fig:approach-overview}
\end{figure}
As previously discussed, treating the integration duration $\tau$ as coordinate is inefficient and makes the learning process more difficult. Thus, proper treatment of the $\tau$ variable is a necessity. To this end, we propose an architecture design that allows to satisfy the identity property by design and at the same time yields a very simple gradient network when $\tau = 0$. Let us consider an arbitrary INR:-
\begin{equation}
    f_{\theta}(\mathbf{x}, t): \mathbb{R}^n \times \mathbb{R} \rightarrow \mathbb{R}^d,
\end{equation}
where $x, t$ are the spatial position and time respectively, $n$ represents the spatial dimension and $d$ represent some latent dimension. Then our proposed architecture uses the following set of operations to satisfy the flow map properties :-
\begin{equation}
\label{eq:pe}
    z_0 = f_{\theta}(\mathbf{x}, t)
\end{equation}
\begin{equation}
\label{eq:residual}
    z_{i+1} = z_{i} + \tau\cdot\psi(W_i z_{i}) 
\end{equation}
\begin{equation}
\label{eq:output}
    \phi_{\theta}(\mathbf{x}, t, \tau) = \mathbf{x} + (W_l z_{l-1}) ,
\end{equation}
where $\psi$ represents an arbitrary activation function which evaluates to 0 when the input is 0 (for example $relu$ activation function). $W_i \in \mathbb{R}^{d \times d}$ for $i < l$ represents the weight matrix of a shallow MLP and $W_l \in \mathbb{R}^{d \times n}$ is the weight matrix for the output layer of the MLP. Clearly, when $\tau = 0$, then the network $\phi_{\theta}(\mathbf{x},t,0) = x$, thereby satisfying the identity property. Additionally,$\frac{\partial\phi_{\theta}(\mathbf{x},t,\tau)}{\partial\tau}$ evaluates to $W_l f_{\theta}(\mathbf{x},t)$ when $\tau = 0$ (Please refer the appendix for the detailed evaluation of the partial derivative). This allows us to learn the vector field parameterized by $f_\theta$, assuming access to ground truth vectors for supervision.

\subsubsection{Flow map self-supervision for efficient learning}
\label{sec:self_supervision}
Learning a flow map representation using flow map samples as supervision requires generation of tremendous amount of ground truth flow map samples. It is unclear how many samples are sufficient for efficient learning and will indeed vary based the on the size and complexity of the dataset. However, optimizing for the vectors is a more feasible option. To this end, we utilize our proposed network architecture which allows us to learn the vector field as a first step using the gradient network $f_\theta$ resulting from $\frac{\partial \phi_\theta}{\partial\tau}$ when $\tau = 0$. What remains next is to learn flow maps when $\tau > 0$. To achieve this, we take advantage of the flow map compositions. To understand flow map composition, let us consider a finite time-span $T \in [t_0,t_n]$. Now, dividing the time-span into 2 discrete intervals give us $[t_0, t_1, t_n]$ such that $t_1-t_0 = t_n-t_{1} = t_s$. We can now define flow map composition as follows:-
\begin{equation}
    \phi(\mathbf{x}, t_0, t_n-t_0) = \phi(\phi(\mathbf{x}, t_0, t_s), t_1, t_s))
\end{equation}
Please Note that, the right hand side of the above equation can be composed using any number of intervals, also, the intervals does not necessarily needs to be equally spaced. We take advantage of this specific composition property of flow maps to learn neural flow maps $\phi_\theta(x, t, \tau)$ for $\tau > 0$ in the form of self-supervision. The basic idea behind this approach is that, we first learn a good approximation of the vector field as a consequence of Eq.~\ref{eq:zero_tau_deriv} using $f_\theta$. We assume that, for small non-zero $\tau$ value we can obtain good approximation for the instantaneous motion as a result of the inductive bias of the neural network. Thereby, we employ the following self-supervised composition loss to learn the flow maps at $\tau > 0$:-
\begin{equation}
\label{eq:composition}
    || \frac{\partial \phi_{\theta}(\mathbf{x}, t, \tau_n)}{\partial \tau} - \frac{\partial\phi_\theta(\phi_\theta(\phi_\theta(x, t, \tau_{n1}), t+ \tau_{n1}, \tau_{n2}), t+ \tau_n, 0)}{\partial \tau}||_2,
\end{equation}
where, $n1 + n2 = n$. Note in practice, multiple numbers of composition steps are taken to get a more accurate flow map prediction. Since, we have only optimized for the instantaneous vectors, it is unreasonable to expect good prediction of flow map at $\tau = \tau_n$, however, by taking multiple composition steps with sufficiently small $\tau$ values we can expect reasonably good approximation for the right hand side of the equation with increasing optimization steps.


\section{Network Architecture}
\begin{figure*}[!t]
  \centering
 	\includegraphics[width=\linewidth]{figures/illustrative_network.pdf}
	\caption{TODO}
    \label{fig:illustrative_network}
\end{figure*}
In this section, we describe network architecture in details and provide justification for the choices we made.

Our overall architectural design follows the set of operations described in Sec.~\ref{sec:neural_flow_map}. More specifically, we use the localized Grid-SIREN similar to the one's used in previous works ~\cite{} as our choice of $f_\theta$. However, we want to learn the flow maps in a two-stage process (1) learning the vector field at $\tau=0$ as described in Sec.~\ref{sec:learning_vf} and (2) learning the flow maps for $\tau>0$ as described in Sec.~\ref{sec:self_supervision}. Thus, having the same set of learnable frequencies in the form of a single feature grid responsible for both learning the vector field as well as flow maps for $\tau > 0$ can possibly impact the optimization process negatively. To this end, we propose a decoupled split architecture wherein $f_\theta$ is designed to be comprised of two separate components, enabling us to learn the vector field and the flow maps when $\tau > 0$ without any entanglement. 

\textbf{Decoupled Split Architecture} Let us denote the two decoupled components of $f_\theta(\mathbf{x}, t, \tau)$ as $g_\theta(\mathbf{x}, t, \tau)$ and $h_\theta(\mathbf{x}, t, \tau)$ respectively. We use the localized feature grids as positional encoding for both $g_\theta$ and $h_\theta$, whose combined size depends on the input dimensionality $d_i$ of the time-varying vector field. For examples, for $d_i = 3$ i.e. a 2-d time-varying vector field the combined size of the feature grids amounts to $Z \subset \mathbb{R}^{D \times w \times h \times t}$, where $D$ denotes the feature dimensions (the number of learnable frequencies), $w, h,$ and $t$ denotes the width, height and temporal dimension of the discretized vector field. We split the total size of $Z$ into two equal parts resulting in two feature grids $Z_g$ and $Z_h$. We then form $g_\theta$ using $Z_g$ as the positional encoding, followed by a linear layer mapping and an non-linear activation to get a latent vector $l_g$. We then scale the latent vector by the input $\tau$ value multiplied by a learnable scalar $\tau_{pe}$. To summarize we obtain the latent vector $l_g$ as output of the first component $g_\theta$ using the following operations:-
\begin{equation}
    l_g = (\tau * \tau_{pe})\cdot \psi(W_0\ interp(\mathbf{x}, t, Z_g)),
\end{equation}
where, $\psi$ represents non-linear activation function. In practice, we use swish activation function unless otherwise specified.
We obtain another latent vector $l_h$ as the output of $h_\theta$ which corresponds to the second component of $f_\theta$. We form $h_\theta$ by using $Z_h$ as positional encoding, followed by a linear layer mapping. The latent vector $l_h$ is obtained through the following operation:
\begin{equation}
    l_h = \hat{W}\ interp(\mathbf{x}, t, Z_h)
\end{equation}
We then form $f_\theta$ as a combination of $g_\theta$ and $h_\theta$ using the following operation:-
\begin{equation}
    f_\theta = \psi(W_f\ \tanh(l_g) * l_h)
\end{equation}
After $f_\theta$ is obtained we use a shallow 3-layer MLP and follow the same set of operations described in Eq.~\ref{eq:residual} and~\ref{eq:output}. Using out decoupled split architecture we can efficiently learn the vector field in the first stage of optimization by utilizing $g_\theta$ and during the second stage learn the flow maps for $\tau > 0$ using $h_\theta$.

\section{Optimization}
\begin{figure}
  \centering
 	\includegraphics[width=0.7\linewidth]{figures/optimization.pdf}
	\caption{TODO}
    \label{fig:optim}
\end{figure}
We employ a two-stage optimization process to efficiently learn the neural flow map representation without requiring ground truth flow map samples as supervision. In the first stage of optimization we aim to optimize for the vector field by minimizing the following loss function:-
\begin{equation}
    \frac{1}{|\mathbb{T}|} \sum || \frac{\partial \phi_\theta(\mathbf{x}, t, 0)}{\partial \tau} - f(\mathbf{x},t) ||_2
\end{equation}
where, $\mathbb{T}$ represents the total number of ground truth vectors. Please note that, $\frac{\partial \phi_\theta(\mathbf{x}, t, 0)}{\partial \tau}$ corresponds to following set of operation in our architecture:-

\begin{equation}
    z_0 = \tau_{pe}\cdot \psi(W_0\ interp(\mathbf{x}, t, Z_g))    
\end{equation}

\begin{equation}
    z_{out} = z_0\ W_f^T    
\end{equation}
As a consequence of this optimization process, the feature grid $Z_g$ where the bulk of the network parameters for $f_\theta$ exists captures the instantaneous vectors. After optmizing for the vector field, in the second stage of optimization we aim to learn the flow maps for $\tau > 0$.
Assuming, we were able to learn a good approximation of the vector field, we utilize the self-supervision loss as described in Sec.~\ref{sec:self_supervision} to learn flow maps for $\tau > 0$. Please note that at the beginning of the second stage of optimization, we have good approximation of instantaneous vectors, however, for larger $\tau$ value the network is expected to be inaccurate. Thus, composing flow maps by taking multiple steps with sufficiently small $\tau$ values can provide a good approximation and act as a supervision for the single step flow map (left hand side of Eq.~\ref{eq:composition}). However, this limits us from optimizing for extremely large $\tau$ values. Thus, for the second stage of optimization we choose a $\tau_{max}$ and sample $\tau_m < \tau_{max}$ uniformly at random for optimization. Additionally, during the second stage of training we use a different optimizer for $f_\theta$ and set a low learning rate to avoid significant changes to the already learned vector field and only fine-tune the parameters.


==> old-results.tex <==
We first evaluate our method qualitatively for various 2D time-varying datasets. In Fig.~\ref{fig:ftle_fluid} we compare the FTLE generated using our technique and the baseline techniques. We can see that our technique is superior in terms of the visual quality of the FTLE. Both SIREN and Super-resolution show artifacts which manifests in different forms for both the cases. For the super-resolution method, grid-artifacts resulting from the use of convolutional layers appear quite prominently. On the other hand, our technique is able to produce a FTLE with no significantly visible artifacts and is able to capture the ridges quite well. In Fig.~\ref{fig:ftle_dg}, ~\ref{fig:ftle_cy} and~\ref{fig:ftle_bo} we show additional FTLE results for the double gyre, flow over cylinder and the boussinesq dataset for various other baselines. We can clearly see the shortcomings of the Encoder-Decoder network architecture from the FTLE results for the flow over cylinder and boussinesq dataset. Clearly, the network failed to learn a good approximation of the flow maps, we suspect this is largely due to (1) the complexity of the datasets, (2) the absence of positional encoding in the network design which has been shown in the literature~\cite{tancik2020fourier, sitzmann2020implicit}, to help capture high frequency details present in the data, and (3) the network design failing to satisfy the basic properties of the flow map described in Sec.~\ref{sec:integrationfree}. Similarly, the comparatively poor results of a SIREN is the consequence of the network not being able to satisfy the flow map properties. For fair comparison both SIREN and the Encoder-Decoder networks were trained with the same amount of data our technique was trained on. We further show comparison with Spline Interpolation technique by Li et al. Please note that, to fit the splines we provide the method with a very dense sampling of pathlines by integrating particles with the same starting time and time-span as the query pathlines. More specifically, we seed $3\times$ the total spatial resolution of the dataset uniformly at random at the starting time and then generate pathlines. The start time and the time span of the pathlines aligns with the start time and time span of the query pathlines. This allows the technique to utilize a better distribution of particles, and thus a better neighborhood for query interpolation. Alternatively, if the lagrangian representation consists of particles starting at some arbitrary time much earlier than the query start time the quality of the FTLE generated degrades significantly for the flow over cylinder and boussinesq dataset. Additionally, we also evaluate our method quantitatively for 2D time-varying datasets. Fig.~\ref{fig:quantitative} shows the error between the ground truth flow maps and the predicted flow maps for different method across different datasets. We vary the starting times and flow map duration to show the change in error for datasets that becomes increasingly complex over time. The flow map error reported is computed as the euclidean distance between the ground truth flow map and the predicted flow map with respect to the bounding box diagonal. We can see that our network achieves lower error comparatively against all the method across most of the datasets. The only exception being the Boussinesq dataset wherein the Spline Interpolation outperforms our technique. Given the distribution of samples and the number of pathlines splines were fit to, makes the task of interpolation for new trajectories easier and gives the technique an advantage over our technique. However, the low error comes at a cost of higher computational cost. 

In Table~\ref{tab:time}, we show the training/fitting to the spline times for the our technique and other baselines as well the inference times for generating flow maps. We can see that our technique has the fastest inference time when compared to all the other baselines. Please note that, the inference time reported for the flow map super-resolution technique includes the CNN-network inference time as well as the time required to compute the low-resolution flow map which is the input to the network. We argue that even though the network inference time is fast, the network still requires the computation of a  low-resolution flow map to generate the high-resolution one. The computation cost of generating the low-resolution flow map is not negligible and thus, should be taken into consideration for fair comparison to our method which does not rely on any additional information during the inference time. We can see that the B-spline curve fitting time is incredibly fast as compared to our training time. However, this fast fitting time for Spline interpolation has little bearing on the inference time, which can get really slow depending on the number of pathlines the B-splines curves were fit to and the total number of query pathlines. On the contrary, our method scales well to the large number of query pathlines and maintains a fast inference time across all the dataset.
